Highly Optimized Full-Core Reactor Simulations on Summit

Nek5000/RS is a highly-performant open-source spectral element code for simulation of incompressible and low-Mach fluid flow, heat transfer, and combustion with a particular focus on turbulent flows in complex domains. It is based on high-order discretizations that realize the same (or lower) cost per gridpoint as traditional low-order methods. State-of-the-art multilevel preconditioners, efficient high-order time-splitting methods, and runtime-adaptive communication strategies are built on a fast OCCA-based kernel library, libParanumal, to provide scalability and portability across the spectrum of current and future high-performance computing platforms. On Summit, Nek5000/RS has recently achieved an milestone in the simulation of nuclear reactors: the first full-core computational fluid dynamics simulations of reactor cores, including pebble beds with > 350,000 pebbles and 98M elements advanced in less than 0.25 seconds per Navier-Stokes timestep. With carefully tuned algorithms, it is possible to simulate a single flow-through time for a full reactor core in less than six hours on all of Summit.

==> tex/preambl.tex <==

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Geometry 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%\usepackage{geometry}
%\geometry{left   = 1.0in,
%          right  = 1.0in,
%          top    = 1.0in,
%          bottom = 1.0in}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Formats
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%\usepackage{arydshln}
\usepackage[utopia]{mathdesign}
\usepackage{textcomp}
\usepackage{comment}
\usepackage{subfig,pgfplots,epsf,graphicx,color}
\usepackage{amsmath,amsfonts,amsthm,multirow}

%\usepackage[demo]{graphicx}
\usepackage{rotating}
\usepackage{tabularx}
\usepackage{float}

\usepackage{pdfpages}
\usepackage{afterpage}
\usepackage{wrapfig}
\usepackage{microtype}
\usepackage{fullpage}
\usepackage{bm} 
\usepackage{caption} 
%\usepackage{url}
%\usepackage[hidelinks]{hyperref}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Colors
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\usepackage[colorlinks=true]{hyperref}
\hypersetup{
  colorlinks  = true, %Colours links instead of ugly boxes
% urlcolor    = black, %Colour for external hyperlinks
% linkcolor   = black, %Colour of internal links
% citecolor   = black, %Colour of citations
  urlcolor    = blue, %Colour for external hyperlinks
  linkcolor   = blue, %Colour of internal links
  citecolor   = blue, %Colour of citations
}

\DeclareGraphicsExtensions{.gif,.png,.jpg,.pdf,.tiff,.eps}	
%\DeclareTextCommandDefault{\textcopyright}{\textcircled{c}}
%\DeclareTextCommandDefault{\textregistered}{\textcircled{%
% \check@mathfonts\fontsize\sf@size\z@\math@fontsfalse\selectfont R}}


